Towards a framework on tabular synthetic data generation: a minimalist approach: theory, use cases, and limitations

We propose and study a minimalist approach towards synthetic tabular data generation. The model consists of a minimalistic unsupervised SparsePCA encoder (with contingent clustering step or log transformation to handle nonlinearity) and XGboost decoder which is SOTA for structured data regression and classification tasks. We study and contrast the methodologies with (variational) autoencoders in several toy low dimensional scenarios to derive necessary intuitions. The framework is applied to high dimensional simulated credit scoring data which parallels real-life financial applications. We applied the method to robustness testing to demonstrate practical use cases. The case study result suggests that the method provides an alternative to raw and quantile perturbation for model robustness testing. We show that the method is simplistic, guarantees interpretability all the way through, does not require extra tuning and provide unique benefits.

==> algorithms/PCAICA.tex <==
\begin{figure*}
\begin{minipage}{0.6\linewidth}
\begin{algorithm}[H]
  \caption{ICA}
\hspace*{\algorithmicindent} \textbf{Input}: Data Matrix $Y$\\
\hspace*{\algorithmicindent} \textbf{Output}: $X_{ica}$ rows as independent as possible. 
\begin{algorithmic}[1] \\
In the general matrix setting, $Y=W_{ica}X_{ica}$. The rows of $X_{ica}$ are maximally independent (ground truth independence).
\begin{equation}
    Y=\mu_Y \mathbbm{1}^T+U\Sigma V^H
\end{equation}
$\mu_Y$ is the mean column vector. Apply ICA to $V^H$ (iterative kurtosis maximization) that is obtained via SVD on $Y-\mu_Y \mathbbm{1}^T$. Then, $V^H=Q_{ica} V_{ica}^H$ where $Q_{ica}$ contains the columns of orthogonal components that iteratively maximizes the kurtosis objective.
Writing out   $Y=\mu_Y \mathbbm{1}^T+ U\Sigma Q_{ica} V_{ica}^H$. We can make the identification with $Y=W_{ica}X_{ica}$, with $W_{ica}= U\Sigma Q_{ica}, X_{ica}=W_{ica}^{-1} \mu_Y \mathbbm{1}^T+V_{ica}^H$.
Note, ICA factorization is non-unique: $Y=(W_{ica} D)(D^{-1} X_{ica} )$  
\end{algorithmic}
\label{alg:ica}  
\end{algorithm}
\end{minipage}\hfill
\begin{minipage}{0.33\linewidth}
\begin{algorithm}[H]
  \caption{PCA}
\hspace*{\algorithmicindent} \textbf{Input}: Data Matrix $Y$\\
\hspace*{\algorithmicindent} \textbf{Output}: $X_{pca}$ rows as uncorrelated as possible. 
\begin{algorithmic}[1]  \\
In the general matrix setting,
\begin{equation}
 Y=W_{pca} X_{pca}	    
\end{equation}
The rows of $X_{pca}$ are maximally uncorrelated. With a similar decomposition,
\begin{equation}
    Y=\mu_Y \mathbbm{1}^T+U\Sigma V^H
\end{equation}
We have $W_{pca}= U\Sigma, X_{pca}=(U\Sigma)^{-1} \mu_Y \mathbbm{1}^T+V^H$.


\end{algorithmic}
\label{alg:pca}  
\end{algorithm}
\end{minipage}
\end{figure*}

==> algorithms/TSNE.tex <==
\begin{figure*}
\begin{minipage}{\linewidth}
\begin{algorithm}[H]
  \caption{tSNE}
\hspace*{\algorithmicindent} \textbf{Input}: Input data matrix $\pmb{X}\in \mathbbm{R}^{n\times p}$, Perplexity factor $PP\in \mathbbm{R}_{+}$, Initialization variance $\sigma$ \\
\hspace*{\algorithmicindent} \textbf{Output}: Output data matrix embedding $\pmb{Z}\in \mathbbm{R}^{n\times p'}$, $2 \leq p'\ll p$ 
  \begin{algorithmic}[1]\\
\begin{itemize}
    \item \textit{Construct summary statistics in raw data dimensions}
\end{itemize}
\noindent\textbf{For each}$(i,j)$\textbf{compute}\quad 
    $ p_{{\color{Cerulean}{j}}\mid {\color{ForestGreen}{i}}} = \frac{e^{\frac{-\|x_{\color{Cerulean}{j}}-x_{{\color{ForestGreen}{i}}}\|^2}{2\sigma_{\color{ForestGreen}{i}}^2}}}{
       \sum_{k\neq {\color{ForestGreen}{i}}} e^{\frac{-\|x_{\color{ForestGreen}{i}}-x_k\|^2}{2\sigma_{\color{ForestGreen}{i}}^2}}
       }$,   \algorithmiccomment{Numerator: joint, Denominator: marginal, $p_{i\mid i}=0 $ vacuous}\\\algorithmiccomment{
       The Gaussianity factor $\sigma_i$ being obtained from solving equation $PP(p_{j\mid i}(\sigma_i))\equiv PP(\sigma_i)=PP$ between the   perplexity derived from the conditional probabilities and the user defined perplexity factor $PP$. Namely, $PP(p)\equiv 2^{H(p)}\equiv 2^{\mathbbm{E}[\log_2 p]}$,  $PP(p_{j\mid i}(\sigma_i))\equiv 2^{-\sum_j p_{j\mid i}\log_2 p_{j\mid i}}$ }\algorithmiccomment{$p_{j\mid i}$: Picking $j$ amongst all the neighbors of $i$}\\\algorithmiccomment{Suggested $PP$ values are between 5 and 50 \cite{van2008visualizing}, but need careful analysis depending on data}  \\\algorithmiccomment{Higher perplexity may often enforce meaningful topologies (non-local information preserved) and clearer clusters}
      
     \noindent\textbf{Obtain} the symmetrized measure $p_{ij}=\frac{p_{j\mid i}+p_{i\mid j}}{2n}$ \algorithmiccomment{Put $i$ and $j$ on the same footing}\\

\begin{itemize}
    \item \textit{Minimize the deviation between the structure of ``ground truth'' $p_{ij}$ and target $q_{ij}$}
\end{itemize}\\
\textbf{Set up} the target similarity measure $q_{ij}=\frac{(1+\|z_i-z_j\|^2)^{-1}}{\sum_{l\neq k}(1+\|z_k-z_l\|^2)^{-1}}$ from $t$ distribution with 1 degree of freedom\\\algorithmiccomment{While $p_{ij}$ was roughly constructed from gaussian, $q_{ij}$ derives from t distribution $t_{\nu}\equiv t_{1}\equiv\text{Cauchy}$}\\
\algorithmiccomment{ The heavy-tailedness of t-distribution allow dissimilar objects separate apart into the tails.}\\
     \textbf{Initialize} $\pmb{Z}\equiv (z_1,z_2,...,z_N)$ according to multivariate normal distribution $y_i\sim \mathcal{N}(0,\sigma^2)$ \\
     \textbf{Optimize} the KL divergence $\min_{q}KL(P||Q)=\sum_{i\neq j}p_{ij}\log\frac{p_{ij}}{q_{ij}}$ via gradient descent and obtain $\pmb{Z}$   
\end{algorithmic}
\label{alg:tsne}  
\end{algorithm}
\end{minipage}
\end{figure*}

==> algorithms/UMAP.tex <==
\begin{figure*}
\begin{minipage}{\linewidth}
\begin{algorithm}[H]
  \caption{UMAP}
  \hspace*{\algorithmicindent} \textbf{Input}: Input data matrix $\pmb{X}\in \mathbbm{R}^{n\times p}$, Nearest neighbor factor $k$, distance metric choice $d(\cdot,\cdot)$, Minimial distance in low dimensional space $d_{\min}$ \\
 \hspace*{\algorithmicindent} \textbf{Output}: Output data matrix embedding $\pmb{Z}\in \mathbbm{R}^{n\times p'}$, $2 \leq p'\ll p$ 
  \begin{algorithmic}[1]\\
\begin{itemize}
    \item \textit{Construct k-nearest weighted graph layout in raw data dimensions}
\end{itemize}
\\
\textbf{Find} the $k-$nearest neighbor for every observation $x_1,x_2,...,x_n$  according to the distance metric $d(\cdot,\cdot)$. Denote the set as $\{x_{i_1},....x_{i_k}\}$\\
\textbf{Select } the proper parameter $\sigma_i$ for each observation $i$ similar to tSNE perplexity factor calibration on $\sigma_i$.\\
\begin{equation}
    \log_2 (k) = \sum_{j=1}^k \exp\Big(\frac{-\max\{0,d(x_i,x_{i_j})-\rho_i\}}{\sigma_i}\Big)
\end{equation}
where $\rho_i$ is the minimal distance to a neighbor in the data i.e., $\rho_i = \min\{d(x_i,x_j)\mid 1\leq j \leq n, j\neq i,  d(x_i,x_j)>0\} $\\\algorithmiccomment{Since there exists a Riemannian metric where data distributes uniformly\cite{mcinnes2018umap}, one creates a custom metric to ensure the uniformity. The RHS is the sum of smoothed nearest neighbor distances similar to the Gaussian prior in tSNE.}\\\algorithmiccomment{$\sigma_i$ normalize the distances across observations and its neighbors and ($\rho_i$,$\sigma_i$) correspond to local Riemannian metric.}\\
\textbf{Construct} the weights by the weight functions $w(x_i,x_{i_j})=\exp\Big(\frac{-\max\{0,d(x_i,x_{i_j})-\rho_i\}}{\sigma_i}\Big)$, where $\sum_{j=1}^kw(x_i,x_{i_j})=log_2(k)$\\
\textbf{Symmetrize} the matrix by putting $w_{i\leftrightarrow j}=w(x_i,x_j)+w(x_j,x_i)-w(x_i,x_j)\cdot w(x_j,x_i)$, the edge (hence the weights) exists only if $i$ is the $k-$nearest neighbor of $j$ or vice versa.\\
\begin{itemize}
    \item \textit{Optimize for the low dimension layout using \underline{force-directed graph layout}}
\end{itemize}
\\
\textbf{Initialize } the output $\pmb{Z}$ using spectral embedding.\\\algorithmiccomment{Symmetric Laplacian $G$ is a discrete Laplace-Beltrami operator of the manifold}\\
\textbf{Optimize } for the structure for the edges $(i,j)$ in the graph $G$ by applying \textit{attracting} and \textit{repulsive} force as following (the process is done by iterating over the edges in $G$):
\\
\begin{enumerate}
    \item \underline{\textbf{Attractive force}}: Attract $i$ to $j$
    \begin{equation}
        z_i = z_i +\alpha\cdot\frac{-2ab\|z_i-z_j\|_2^{2(b-1)}}{1+a(\|z_i-z_j\|_2^2)^b}w_{i\leftrightarrow j}(z_i-z_j)
    \end{equation}
     \algorithmiccomment{$a,b$ are fitted via Nonlinear least squares $\frac{1}{(1+a\|z_i-z_j\|_2^{2b})}$(for differentiable update) to $\exp\Big(\frac{-\max\{0,d(x_i,x_{i_j}-\rho_i)\}}{\sigma_i}\Big)$.}
    \item \underline{\textbf{Repulsive Force}}: Repulse $i$ from $k$, where $k$ is sampled from non-neighboring vertices.
    \begin{equation}
        z_i = z_i+\alpha\cdot \frac{b}{(\epsilon+\|z_i-z_k\|_2^2)(1+a(\|z_i-z_k\|_2^{2b}))}(1-w_{i\leftrightarrow j})(z_i-z_k)
    \end{equation}
\end{enumerate}
\algorithmiccomment{$\epsilon$ is a small number clips away numerics that is close to 0 in the denominator }
\end{algorithmic}
\label{alg-umap}
\end{algorithm}
\end{minipage}
\end{figure*}


==> algorithms/gradient_boost.tex <==
\begin{figure*}
\begin{minipage}{\linewidth}
\begin{algorithm}[H]
  \caption{Gradient boosting}
  \hspace*{\algorithmicindent} \textbf{Input}: Input training $\{(x_i,y_i)\}_{i=1}^n$, Iterations: $M$ Objective function $L(y,F(x))$ \\
 \hspace*{\algorithmicindent} \textbf{Output}: Output predicted function form $F_M$ 
  \begin{algorithmic}[1]\\
\begin{itemize}
    \item \textit{Initialize the model $F_0$ with constant value (e.g. mean of the column) }
\end{itemize}
\begin{equation}
    F_0(x) = {\arg\min}_{\tilde{y}}\sum_{i=1}^n L(y_i,\tilde{y})
\end{equation}
\\
\begin{itemize}
    \item \textit{For iterations from 1 to M}
\end{itemize}
\\
\textbf{Compute} the \textit{pseudo-residuals}:
\begin{equation}
    r_{im} = -\Big[\frac{\partial L(y_i,F(x_i))}{\partial F(x_i)}\Big]_{F(x)=F_{m-1}(x)}, \text{ for } i = 1,2,...,n
\end{equation}
\algorithmiccomment{in the MSE example, $L=\sum_{i=1}^n(y_i-F(x_i))^2$, $r_{im}=y_i-F(x_i)$}\\
\textbf{Fit} a base learner (eg. tree) $h_m$ to the pseudo residuals, i.e., fit on the residuals $\{(x_i,r_{im})\}_{i=1}^n$:
\\
\textbf{Compute} the multiplier (learning rate) by solving
\begin{equation}
    \gamma_m =\arg\min_{\gamma} \sum_{i=1}^n L(y_i,F_{m-1}(x_i)+\gamma h_m(x_i))
\end{equation}\\
\textbf{Update} the model
\begin{equation}
    F_m(x) = F_{m-1}(x)+\gamma_mh_m(x)
\end{equation}
\begin{itemize}
    \item \textit{Output $F_M$}
\end{itemize}
\end{algorithmic}
\label{alg:gb}
\end{algorithm}
\end{minipage}
\end{figure*}

